A Machine Learning Framework to Deconstruct the Primary Drivers for Electricity Market Price Events

Power grids are moving towards 100% renewable energy source bulk power grids, and the overall dynamics of power system operations and electricity markets are changing. The electricity markets are not only dispatching resources economically but also taking into account various controllable actions like renewable curtailment, transmission congestion mitigation, and energy storage optimization to ensure grid reliability. As a result, price formations in electricity markets have become quite complex. Traditional root cause analysis and statistical approaches are rendered inapplicable to analyze and infer the main drivers behind price formation in the modern grid and markets with variable renewable energy (VRE). In this paper, we propose a machine learning-based analysis framework to deconstruct the primary drivers for price spike events in modern electricity markets with high renewable energy. The outcomes can be utilized for various critical aspects of market design, renewable dispatch and curtailment, operations, and cyber-security applications. The framework can be applied to any ISO or market data; however, in this paper, it is applied to open-source publicly available datasets from California Independent System Operator (CAISO) and ISO New England (ISO-NE).

==> tables/caiso_results.tex <==
\begin{table}[]
    \centering
    \caption{Caption}
    \label{tab:my_label}
    \ra{1.3}
    \resizebox{\columnwidth}{!}{\%
    \begin{tabular}{llll}
    \toprule
     \multirow[c]{7}{*}{Congestion (146, 60\%)} &  & \multirow[c]{2}{*}{PGAE (106, 43\%)} & Avg (4, 2\%)\\
     &  &  & Mov (104, 43\%)\\
     &  & \multirow[c]{2}{*}{SCE (54, 22\%)} & Avg (8, 3\%)\\
     &  &  & Mov (47, 19\%)\\
     &  & SDGE (6, 2\%) & Mov (6, 2\%)\\
     &  & \multirow[c]{2}{*}{VEA (120, 49\%)} & Avg (2, 1\%)\\
     &  &  & Mov (119, 49\%)\\  \hline
    \multirow[c]{2}{*}{Day Ahead (32, 13\%)} & Congestion (5, 2\%) & SCE (5, 2\%) & Avg (5, 2\%)\\
     & Energy (28, 11\%) & PGAE (28, 11\%) & Avg (28, 11\%)\\  \midrule
    Demand (13, 5\%) &  (13, 5\%) &  (13, 5\%) & Avg (13, 5\%)\\  \hline
    \multirow[c]{7}{*}{Forecasting Error (110, 45\%)} & \multirow[c]{5}{*}{Ver (99, 41\%)} & \multirow[c]{2}{*}{Dam (63, 26\%)} & Avg (16, 7\%)\\
     &  &  & Mov (51, 21\%)\\
     &  & Rtd (4, 2\%) & Avg (4, 2\%)\\
     &  & \multirow[c]{2}{*}{Rtpd (52, 21\%)} & Avg (14, 6\%)\\
     &  &  & Mov (41, 17\%)\\
     & \multirow[c]{2}{*}{Demand (21, 9\%)} & \multirow[c]{2}{*}{Dam (21, 9\%)} & Avg (12, 5\%)\\
     &  &  & Mov (9, 4\%)\\  \hline
    \multirow[c]{8}{*}{Generation (122, 50\%)} & \multirow[c]{2}{*}{Non-Renewables (24, 10\%)} & Nuclear (4, 2\%) & Mov (4, 2\%)\\
     &  & Thermal (20, 8\%) & Mov (20, 8\%)\\
     & \multirow[c]{6}{*}{Renewables (105, 43\%)} & \multirow[c]{2}{*}{Large.Hydro (64, 26\%)} & Avg (39, 16\%)\\
     &  &  & Mov (29, 12\%)\\
     &  & \multirow[c]{2}{*}{Non-Ver (16, 7\%)} & Avg (11, 5\%)\\
     &  &  & Mov (5, 2\%)\\
     &  & \multirow[c]{2}{*}{Ver (37, 15\%)} & Avg (24, 10\%)\\
     &  &  & Mov (13, 5\%)\\  \hline
    \multirow[c]{3}{*}{Regulation Prices (41, 17\%)} & \multirow[c]{3}{*}{ (41, 17\%)} & Rd (1, 0\%) & Avg (1, 0\%)\\
     &  & Rmd (1, 0\%) & Mov (1, 0\%)\\
     &  & Ru (40, 16\%) & Mov (40, 16\%)\\
     \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/data.tex <==
\begin{table}
    \centering
    \caption{Data Description}
    \label{tab:lodes}
    \scriptsize
    %\begin{tabular}{|l|p{2cm}|p{2cm}|p{2cm}|}
    \begin{tabular}{|p{1.5cm}|p{1.8cm}|p{1.75cm}|p{2cm}|}
    \toprule
    Parameter & Common Variables & CAISO & ISONE \\ [0.5ex] 
    \midrule
    Prices (P) &  Marginal Cost of Energy ($_{E}$), Marginal Cost of Congestion ($_{C}$) &  & \\ \midrule
    Generation (G) &  Nuclear ($_N$), Hydro ($_H$) & Thermal ($_T$), VER ($_{VER}$), Other Renewables ($_{OR}$) & Solar ($_S$), Wind ($_W$), Oil ($_O$), Landfill Gas ($_{LG}$), Refuse ($_R$), Wood ($_{Wo}$), Coal ($_C$), Natural Gas ($_{NG}$) \\\midrule
    Demand (D) & Load ($_L$) &  &  \\\midrule
    Forecast Error (FE) & Day-ahead demand ($_{D}$) & VER ($_{VER}$) & Wind ($_W$)\\\midrule
    Reserves (R) &  & Regulation Up ($_{RU}$), Regulation Down ($_{RD}$) &   \\\midrule
    Curtailment (C) &  & Wind ($_W$), Solar ($_S$) & \\\midrule
    Transfers ($T$) & Imports($_I$) & & Exports ($_E$)\\
    \bottomrule
    \end{tabular}
\end{table}
